Towards Complex Text-to-SQL in Cross-Domain Database with Intermediate Representation

We present a neural approach called IRNet for complex and cross-domain Text-to-SQL. IRNet aims to address two challenges: 1) the mismatch between intents expressed in natural language (NL) and the implementation details in SQL; 2) the challenge in predicting columns caused by the large number of out-of-domain words. Instead of end-to-end synthesizing a SQL query, IRNet decomposes the synthesis process into three phases. In the first phase, IRNet performs a schema linking over a question and a database schema. Then, IRNet adopts a grammar-based neural model to synthesize a SemQL query which is an intermediate representation that we design to bridge NL and SQL. Finally, IRNet deterministically infers a SQL query from the synthesized SemQL query with domain knowledge. On the challenging Text-to-SQL benchmark Spider, IRNet achieves 46.7% accuracy, obtaining 19.5% absolute improvement over previous state-of-the-art approaches. At the time of writing, IRNet achieves the first position on the Spider leaderboard.

==> challenges.tex <==
\section{Spider Data Analysis}
\label{sec:challenges}
\input{challenges_statistics_tables}
\input{oov_statistics_tables}

To understand the main challenges in Spider benchmark, we conduct a thorough analysis on it with  SyntaxSQLNet~\citep{Syntaxsqlnet2018}, which is the state-of-the-art approach and achieves $24.8\%$ exact matching accuracy on development set and $27.2\%$ on test set.

\subsection{Setup}
We first evaluate SyntaxSQLNet on development set of Spider in the database split settings.
That is NL specifications under test are over unseen schemas during training.
Then, we manually investigate all the error examples (838 in total), categorize them based on the cause for failures and induce the main challenges.
Unlike the previous study~\citep{Yavuz2018takes} on WikiSQL that only focuses on the \texttt{WHERE} clause, we make a more comprehensive study on the complete SQL. 
We find that most examples have more than one causes for failure.
Hence, if an example belongs to more than multiple categories, we include it in all the categories that can be applyed.

\subsection{Results}
We summarize three main challenges in Spider.
The number of failure examples for these challenges are shown in Table~\ref{tab:challenge_statistics}.
We describe the three challenges below.

\noindent \textbf{Column Prediction.}
There are $64.6\%$ of examples exhibiting challenges in predicting columns.
Specifically, $29.2\%$ of examples fail to predict a correct column, though the column appears in NL with exactly the same surface form in schema.
Such result is surprising since that predicting a column that exactly appears in NL is supposed to be the easiest task.
Besides, $24.3\%$ of examples fail to predict a correct column that partially appears in NL.
$21.0\%$ of examples predict an incorrect column or miss a column in the \texttt{WHERE} clause, because the correct column is not mentioned in the NL but the value belonging to it is mentioned.

The poor performance of SyntaxSQLNet in predicting those columns that are exactly or partially mentioned in NL may be due to the way it encodes columns and the large number of out-of-vocabulary words, or OOV for short.

Specifically, we find that $97.9\%$ database schemas have duplicated column names and 
$24.6\%$ of column names in a schema are duplicatged on average.
To address the problem, SyntaxSQLNet 
constructs a column embedding by running a bidirectional LSTM over its name and the name of its table.
However, we observe that in some examples the table name of a column is not mentioned in NL.
Even if the table-aware column representations in SyntaxSQLNet effectively distinguish duplicated column names, it may cause difficulties in capturing the matching signals between words in NL and columns.
The large number of OOV in Spider may also explain the poor performance, as shown in Table~\ref{tab:oov_statistics}.
For example, $35.0\%$ of words in database schemas of development set do not occur in the schemas of training set.
The OOV may lack of an accurate representations in a trained model, which may make the model challenging to predict columns.

At last, to address the cases where only the value of a column is mentioned,  as the study points out~\citep{Yavuz2018takes}, the content of a database or external knowledge is needed. 

\noindent \textbf{Schema Comprehension.}
$32.8\%$ of examples predict incorrect tables or omit tables that are explicitly mentioned in the NL, especially when the SQL involves a special column `*'.
Considering the example \#1 in Table~\ref{tab:examples}, even though the table `orchestra' is mentioned in the NL, the predicted SQL still omits it in \texttt{FROM} clause.
Such failures stem from the inequality of status between column and table in SyntaxSQLNet.
Table mainly serves as a context for its columns, and the tables involved in a SQL is inferred from the predicted columns.
However, when a special column `*' is selected, it becomes challenging to infer all the tables.
One possible solution to this problem is to explicitly predict the tables.
However, how to let the model learn to understand the complicated relations among tables and the relations between tables and columns,  becomes a challenging problem.
We refer this challenge as Schema Comprehension. 


\noindent \textbf{Mismatch between NL and SQL.}
There are $16.5\%$ of examples that fail to predict the correct column to be grouped by or miss a \texttt{GROUPBY} clause.
However, unlike the Column Prediction challenges discussed above, the column to be grouped by is usually not mentioned in the NL, which makes it challenging for prediction.
Considering the example \#2 in Table~\ref{tab:examples}, the `Orchestra\_ID' is never mentioned in the NL.
Such failures stem from a mismatch between NL and SQL.
Taking the \texttt{GROUPBY} clause as an example, it is introduced in SQL to facilitate the implementation of aggregate functions.
However, intent expressed in an NL would not consider such implementation details.
The distinct characteristics among NL and SQL inevitably leads to such a mismatch between them.
Due to the existence of this mismatch, we hypothesize that directly synthesizing a SQL from an NL may not be the best solution for Text-to-SQL.  


==> challenges_statistics_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
	\footnotesize
	\centering
	\begin{tabular}{l|c|c}
		\hline 
		\multicolumn{1}{l|}{\textbf{Challenges}} & \multicolumn{1}{c|}{\textbf{\# Examples}}   & 
		\multicolumn{1}{c}{\textbf{Percentage}} \\ \hline \hline
		Column Prediction & 541 & 64.6\% \\ \hline
		Schema Comprehension & 275 & 32.8\% \\ \hline
		Mismatch between NL and SQL & 138 & 16.5\% \\ \hline
	\end{tabular}
	\caption{\label{tab:challenge_statistics} The number of examples exhibiting each challenge.}
\end{table}

==> component_matching_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
	\small
	\centering
	\label{tab:component_matching_results}
	\begin{tabular}{l|c|c|c|c|c|c}
		\hline
		\multicolumn{1}{l|}{\textbf{Approach}} & \multicolumn{1}{c|}{\textbf{IR}}   & \multicolumn{5}{c}{\textbf{Test}}   \\ 
		\cline{3-7}
		&  & 
		\multicolumn{1}{c|}{\texttt{SELECT}}        & \multicolumn{1}{c|}{\texttt{WHERE}}        &
		\multicolumn{1}{c|}{\texttt{GROUP BY}}        & \multicolumn{1}{c|}{\texttt{ORDER BY}}        &
		\multicolumn{1}{c}{\texttt{KEYWORDS}}       \\
		\hline \hline
		Seq2Seq & \multirow{7}{*}{SQL} & 13.0\% & 1.5\% & 3.3\% & 5.3\% & 8.7\% \\
		Seq2Seq+Attention && 14.9\% & 2.5\% & 2.0\% & 1.1\% & 4.8\% \\
		Seq2Seq+Copying && 12.0\% & 3.1\% & 5.3\% & 5.8\% & 7.3\% \\
		SQLNet && 26.2\% & 12.6\% & 6.6\% & 1.3\% & 12.4\%  \\
		TypeSQL && 19.6\% & 7.6\% & 3.8\% & 0.8\% & 8.2\% \\
		SyntaxSQLNet && 38.6\% & 17.6\% & 16.3\% & 4.9\% & 19.7\% \\ 
		SyntaxSQLNet (augment) && 48.0\% & 27.0\% & 24.3\% & 4.6\% & 27.2\%  \\ \hline
		Seq2Seq & \multirow{6}{*}{LF} & \% & \% & \% & \% & \% \\
		Seq2Seq+Attention && \% & \% & \% & \% & \% \\
		Seq2Seq+Copying && \% & \% & \% & \% & \% \\
		SQLNet && \% & \% & \% & \% & \% \\
		TypeSQL && \% & \% & \% & \% & \% \\
		SyntaxSQLNet && \% & \% & \% & \% & \% \\
		\hline
		\approach{} & \multirow{5}{*}{LF} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%}  \\
		
		\hspace{2mm}-external knowledge base && \% & \% & \% & \% & \% \\
		\hspace{2mm}-co-attention & & \% & \% & \% & \% & \% \\
		\hspace{2mm}-gate pointer && \% & \% & \% & \% & \%  \\
		\hspace{2mm}-coarse-to-fine && \% & \% & \% & \% & \%  \\
		\hline
		\approach{}(Bert) & LF & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%}  \\
		\hline \hline
	\end{tabular}
	\caption{Component matching results on SQL queries in test set.}
\end{table*}

==> exact_matching_tables.tex <==
% Please add the following required packages to your document 

\begin{table*}[t!]
	\small
	\centering
	\begin{tabular}{l|c|c c c c c|c}
		\hline
		\multicolumn{1}{l|}{\textbf{Approach}} & \multicolumn{1}{c|}{\textbf{IR}}   & \multicolumn{5}{c|}{\textbf{Test}} & \multicolumn{1}{c}{\textbf{Dev}}   \\ 
		\cline{3-8}
		&  & 
		\multicolumn{1}{c}{Easy}        & \multicolumn{1}{c}{Medium}        &
		\multicolumn{1}{c}{Hard}        & \multicolumn{1}{c}{Extra Hard}        &
		\multicolumn{1}{c|}{All}       &
		\multicolumn{1}{c}{All}       \\
		\hline \hline
		Seq2Seq & \multirow{7}{*}{SQL}  & 11.9\% & 1.9\% & 1.3\% & 0.5\% & 3.7\% & 1.9\% \\ 
		Seq2Seq+Attention && 14.9\% & 2.5\% & 2.0\% & 1.1\% & 4.8\% & 1.8\% \\ 
		Seq2Seq+Copying && 15.4\% & 3.4\% & 2.0\% & 1.1\% & 5.3\% & 4.1\% \\
		TypeSQL && 19.6\% & 7.6\% & 3.8\% & 0.8\% & 8.2\% & 8.0\% \\ 
		SQLNet && 26.2\% & 12.6\% & 6.6\% & 1.3\% & 12.4\% & 10.9\% \\
		SyntaxSQLNet && 38.6\% & 17.6\% & 16.3\% & 4.9\% & 19.7\% & 18.9\% \\
		SyntaxSQLNet (augment) && 48.0\% & 27.0\% & 24.3\% & 4.6\% & 27.2\% & 24.8\% \\
		SyntaxSQLNet (Bert) &&  & & & &  & 25.0\% \\

		\hline
		Seq2Seq & \multirow{6}{*}{LF} & \% & \% & \% & \% & \% & 11.4\% \\ 
		Seq2Seq+Attention && \% & \% & \% & \% & \% & 14.7\% \\
		Seq2Seq+Copying && \% & \% & \% & \% & \% & 18.5\% \\
		TypeSQL && \% & \% & \% & \% & \% & 14.4\% \\
		SQLNet && \% & \% & \% & \% & \% & 17.5\% \\
		SyntaxSQLNet && \% & \% & \% & \% & \% & 27.5\% \\ 
		SyntaxSQLNet(Bert) && \% & \% & \% & \% & \% & 28.5\%\\ 

		\hline 

		\approach{} & \multirow{6}{*}{LF} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{53.2\%} \\
		\hspace{2mm}-coarse-to-fine && \% & \% & \% & \% & \% & 51.7\% \\
		\hspace{2mm}-co-attention & & \% & \% & \% & \% & \% & 51.0\% \\
		\hspace{2mm}-input type knowledge && \% & \% & \% & \% & \% & 51.0\% \\
		\hspace{2mm}-column type knowledge && \% & \% & \% & \% & \% & 50.6\% \\
		\hspace{2mm}-gate pointer & & \% & \% & \% & \% & \% & 50.3\% \\
		\hline 
		\approach{}(Bert-base) & \multirow{5}{*}{LF} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{60.3\%} \\
		\hspace{2mm}-coarse-to-fine && \% & \% & \% & \% & \% & 59.9\% \\
		\hspace{2mm}-input type knowledge && \% & \% & \% & \% & \% & 58.3\% \\
		\hspace{2mm}-column type knowledge && \% & \% & \% & \% & \% & 58.2\% \\
		\hspace{2mm}-gate pointer & & \% & \% & \% & \% & \% & 60.6\% \\
		\hline 
		\approach{}(Bert-large) & \multirow{1}{*}{LF} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{61.9\%} \\

		\hline \hline
	\end{tabular}
	\caption{\label{tab:exact_matching_results} Exact matching results on SQL queries with different hardness level.}
\end{table*}

==> experiment_act.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\begin{tabular}{lcc} 
\hline
\multicolumn{1}{l}{\textbf{Methods}}  & \multicolumn{1}{l}{\textbf{ Dev}} \\
\hline
\approach{} &       \\

\hspace{2mm}$-$ w declare column and table  & \textbf{53.3}\% \\
\hspace{2mm}$-$ w/o declare column and table  & 45.5\% \\
\hline \hline
\end{tabular}
\caption{Decoupling column and table on LF}
\label{tab:booktabs}
\end{table}

==> experiment_gate_pointer.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\begin{tabular}{lccc} 
\hline
\multicolumn{1}{l}{\textbf{Approach}}  & \multicolumn{1}{l}{\textbf{ \#Replicate}} & \multicolumn{1}{l}{\textbf{Filter Gain}}  \\
\hline
\approach{}       & 44  & +0.2\%      \\
\hspace{2mm}$-$ gate pointer & 165 & +1.1\% \\
\hline \hline
\end{tabular}
\caption{Gate pointer Experiment}
\label{tab:booktabs}
\end{table}

==> oov_statistics_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
	\small
	\centering
	\begin{tabular}{l|c|c}
		\hline 
		\multicolumn{1}{l|}{\textbf{Corpus}} & \multicolumn{1}{c|}{\textbf{\# Out of domain}}   & 
		\multicolumn{1}{c}{\textbf{Percentage}} \\ \hline \hline
		Question & 673 & 46.1\% \\ \hline
		Database Schema & 114 & 35.0\% \\ \hline
	\end{tabular}
	\caption{\label{tab:oov_statistics} The number of out-of-domain words in question and database schema on the development set of Spider. To be more clear, we do not consider words in the content of a database.}
\end{table}

==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

Our task is as follows: Given a training set of four tuples (NL specification, \lf{}, SQL and schema) $\{(X_i, Z_i, Y_i, S_i)\}^n_{i=1}$, return a SQL synthesizer that takes as input a new NL specification $X$ and a new schema $S$ and outputs SQL $Y$ via logical form $Z$.
Let $x$ denotes a word in $X$, and $s$ denotes a span in $X$, where $X = s_1, s_2, \cdots, s_l$ and $s_i = x_{i1}, x_{i2}, \cdots, x_{ik}$.
A database schema $Z$ is constituted by a set of tables $T$, where $T = \{t_1, t_2, \cdots, t_m\}$. 
Each table $t_i$ contains a set of columns $C_i$, where $C_i = \{c_{i1}, c_{i2}, \cdots, c_{in}\}$.


==> type_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
	\tiny
	\centering
	\begin{tabular}{ll}
		\hline 
		\multicolumn{1}{l}{\textbf{Type of Span and Column}} & \multicolumn{1}{l}{\textbf{Description}} \\ \hline \hline
		\textbf{Span} & \\
		\textsc{Column} & The span exactly or partially matches a column\\
		\textsc{Table} & The span exactly or partially matches a table \\
		\textsc{Value} & The span is likely to be a database value\\
		%\textsc{Comparative} & The word in the span is in comparative form\\
		%\textsc{Superlative} & The word in the span is in superlative form\\
		%\textsc{Aggregate} & An aggregate function is mentioned in the span\\ \hline
		\hline
		\textbf{Column} & \\
		\textsc{Exact Match} & The column is exactly mentioned in NL \\
		\textsc{Partial Match} & The column is partially mentioned in NL \\
		\textsc{Value Exact Match} & A value mentioned in NL exactly links to the column\\
		\textsc{Value Partial Match} & A value mentioned in NL partially links to the column\\ \hline
	\end{tabular}
	\caption{\label{tab:types} The types that the type system will assign to a span in NL and a column in schema.}
\end{table}
